A Trichotomy for Regular Simple Path Queries on Graphs

Regular path queries (RPQs) select nodes connected by some path in a graph. The edge labels of such a path have to form a word that matches a given regular expression. We investigate the evaluation of RPQs with an additional constraint that prevents multiple traversals of the same nodes. Those regular simple path queries (RSPQs) find several applications in practice, yet they quickly become intractable, even for basic languages such as (aa)* or a*ba*. In this paper, we establish a comprehensive classification of regular languages with respect to the complexity of the corresponding regular simple path query problem. More precisely, we identify the fragment that is maximal in the following sense: regular simple path queries can be evaluated in polynomial time for every regular language L that belongs to this fragment and evaluation is NP-complete for languages outside this fragment. We thus fully characterize the frontier between tractability and intractability for RSPQs, and we refine our results to show the following trichotomy: Evaluations of RSPQs is either AC0, NL-complete or NP-complete in data complexity, depending on the regular language L. The fragment identified also admits a simple characterization in terms of regular expressions. Finally, we also discuss the complexity of the following decision problem: decide, given a language L, whether finding a regular simple path for L is tractable. We consider several alternative representations of L: DFAs, NFAs or regular expressions, and prove that this problem is NL-complete for the first representation and PSPACE-complete for the other two. As a conclusion we extend our results from edge-labeled graphs to vertex-labeled graphs and vertex-edge labeled graphs.

==> intro.tex <==
\section{Introduction}
The reachability problem for graphs (finding a path between two nodes) 
represents one of the oldest problems in computer science 
for which very efficient algorithms have been conceived. 
However, for many real-world problems, 
constraints on the path need to be considered and, as a consequence, 
the reachability problem can become computationally hard. 
Problems on regular paths are among the most studied class of constrained path problems.  
In these problems the edge labels along the path must form a word belonging to a given regular language. 
For graph databases, such problems have been considered in the context of regular path queries (RPQs).
Given a language $L$ and two vertices in a database graph,
a regular path query selects pairs of nodes connected by a path whose edge labels form a word in $L$. 
Graph databases and RPQs have been investigated starting from the late 80s
\cite{abit99,barcelo-pods2011,italians1,italians3,italians4,cruz87,fan-icde,guting-graphdb,libkin-icdt2012,mendelzon-simplepath},
and are now again in vogue due to their wide application scenarios,
e.g. in social networks~\cite{socialnetwork-ronen}, 
biological and scientific databases~\cite{leser-biology,biology-olken}, and the Semantic Web~\cite{semantic-web}.
%Due to these new kinds of applications, new query languages and new query paradigms appear 
%by imposing novel challenges to the research community. 
%The fundamental component of a graph database compared to a relational database is the notion of RPQs.
Regular path queries allow to traverse the same nodes multiple times,
whereas regular simple path queries (RSPQs) permit to traverse each vertex only once.
From a theoretical viewpoint, the former notion has overridden the latter, mainly for complexity reasons. 
Indeed, RPQs are computable in time polynomial in both query and data complexity (combined
complexity), while the evaluation of RSPQs is NP-complete   
even for fixed basic languages such as $(aa)^*$ or $a^*ba^*$~\cite{mendelzon-simplepath}.
RSPQs, however, are desired in many application 
scenarios~\cite{leser-biology,biology-olken,barrett-simplepath,leser-largegraphs,JinHWRX10,ward-wireless}, 
such as transportation problems, VLSI design, metabolic networks, DNA matching and routing in wireless networks.
%For instance, users using Google Maps would not like to get trajectories with loops in their 
%results.
%There are two notions of paths: the first, which is known as regular path, allows to 
%traverse the same vertex more than once;
%the second, known as simple (or acyclic) regular path, permits to traverse 
%each vertex only once.
%Even though the latter notion is the classical notion of a path in graph theory, 
%in graph databases it has been fairly less studied than the former.
%This is not surprising, since finding regular simple paths 
%quickly becomes intractable even for basic languages such as $(aa)^*$ or $a^*ba^*$.
%In a general context, pattern queries are often considered as an isomorphism of subgraphs.
As a further example, the problem of finding subgraphs matching a graph pattern can be generalized
to use regular expressions on pattern edges~\cite{fan-icde}. Such queries may also enforce the condition 
that their matched vertices are distinct. 
Additionally, regular simple paths have been recently considered in SPARQL 1.1 queries exhibiting 
property paths. In particular, recent studies on the complexity of property paths in 
SPARQL~\cite{arenas-counting,losemann-sparql} have highlighted the hardness of the semantics proposed by W3C to 
evaluate such paths in RDF graphs. Roughly speaking, according to the semantics considered in~\cite{losemann-sparql}, 
the evaluation of expressions under Kleene-star closure imposes that the involved path is simple, whereas the 
evaluation of the remaining expressions allows to traverse the same node multiple times. As such, 
the semantics studied in~\cite{losemann-sparql} is an hybrid between regular paths 
and regular simple paths semantics.

\noindent \emph{Contributions.}
In this paper, we address the long standing open question~\cite{mendelzon-simplepath,barrett-simplepath}
of characterizing exactly the maximal class of regular languages for which RSPQs are tractable. 
By ``tractable'' we mean computable in time polynomial in the size of the database. 
Precisely, we establish a comprehensive classification of the complexity of RSPQs for a fixed regular language $L$:
given a edge-labeled graph $G$ and two vertices $x$ and $y$, 
is there a simple path from $x$ to $y$ whose edge labels form a word of $L$? 
A first step towards this important issue has been made in~\cite{mendelzon-simplepath}. 
They exhibit a tractable fragment: the class of languages closed by
subword. However, their fragment is not maximal.

Our contributions can be detailed as follows.
%More precisely, we make the following contributions. 
We introduce a class of languages, named $\trC$,  for which RSPQs are computable in
polynomial time, and even in \NL.
We then show that this fragment is maximal 
as the RSPQ problem is \NP-complete for every regular language that does not belong to $\trC$. 
Consequently, we characterize, under the hypothesis $\NL \neq \NP$ that is actually weaker than
$\ptime \neq \NP$, the frontier between tractability and intractability for this problem.
Additionally, $\trC$ also represents the maximal class for which finding a shortest path that satisfies a RSPQ is tractable.
We note that we focus on data complexity as we assume that the language $L$ is fixed. 
At this point, the chart of the classification of the languages is not yet complete.
Therefore, we refine our results to show the following trichotomy: the RSPQ problem is either
\ACzero, \NL-complete or \NP-complete.

% \commentrb{la phrase suivante est elle vraiment utile?}
% When introducing a class of languages (or other objects), 
% a natural question that arises is to give an algorithm that decides whether a given input belongs to the introduced class. 
% In this paper, we thus discuss the complexity to decide, given a language $L$, whether the RSPQ problem for $L$ is tractable.
We discuss the complexity to decide, given a language $L$, whether the RSPQ problem for $L$ is tractable.
We consider several alternative representations of $L$: DFAs, NFAs or regular expressions.
We prove that this problem is \NL-complete for the first representation and \PSPACE-complete for the two others. 

Next, we give a characterization of the tractable fragment $\trC$ for edge-labeled graphs in term of regular expressions.
Moreover, $\trC$ is closed by union and intersection and languages in $\trC$ are aperiodic i.e.
can be expressed by first-order formulas~\cite{schutzenberger65a}.

The above results hold for the common definition of database graphs, i.e. 
edge-labeled graphs. However, it seems natural to take into consideration both queries on top of vertices labels and queries on top of vertices and edges labels.
As an example, a Google Maps user may be interested to specify as a condition a regular expression 
that enforces a stop over in a given city and avoids another city while preferring certain types of 
roads. 
For such a reason, we focus on two other models: vertex-labeled graphs 
or vertex-edge-labeled graphs (where both vertices and edges are labeled). 
Surprisingly, for some languages, the RSPQ problem is simpler on 
vertex-labeled graphs than on edge-labeled graphs. With $L=(ab)^*$ for instance, 
RSPQ is polynomial for vertex-labeled graphs and \NP-complete for edge-labeled graphs. 
Vertex-edge-labeled graphs obviously generalize both edge-labeled graphs and vertex-labeled graphs. 
%and represent the most desirable model since one can express queries exhibiting labels on both edges and vertices. 
Furthermore, we can adapt our results to prove, for these two models, a classification of the same kind as 
the one shown for vertex-labeled graphs: the RSPQ problem is either 
\ACzero, \NL-complete or \NP-complete. 

As a final contribution, we have obtained two minor results. First, we have attempted to study the parametrized complexity of 
tractable RSPQs queries when the parameter is the size of the query. However, we obtained a partial result: we prove that the 
problem is $\FPT$ for the class of finite languages.
Moreover, we prove that the problem is also $\FPT$ for the class of all regular 
languages when the parameter is the size of the path. As a second result, we prove that the problem \spath is polynomial w.r.t. 
combined complexity on  graphs of bounded directed treewidth. This is actually a straightforward generalization of a result of
\cite{directed-treewidth}.
\smallskip

\noindent \emph{Related Work.}
Regular path queries express ways to evaluate regular expression patterns on database graph models
\cite{abit99,barcelo-pods2011,italians1,italians3,italians4,cruz87,fan-icde,guting-graphdb,libkin-icdt2012,mendelzon-simplepath}
or tree-structured models, such as XML~\cite{italians5}.
While the regular path problem has been extensively studied in the literature, 
the regular simple path problem has received less attention in both the database and graph communities.
Besides the works on regular paths, there have been studies on finding paths with some constraints.
In particular, Lapaugh et al.~\cite{lapaugh-evenpath} prove that finding simple paths of even length is polynomial
for non directed graphs and \NP-complete for directed graphs.
This study has been extended in~\cite{arkin-modularity} by considering paths
of length $i\ \mbox{mod}\ k$. 
Similarly, finding $k$ disjoint paths with extremities given as input is polynomial
for non directed graphs~\cite{disjoint-paths-graphs-minors} and \NP-complete for directed graphs~\cite{garey-johnson}.
%Graph queries, expressed in GraphLog \cite{}, represent regular patterns that are ....
Mendelzon and Wood~\cite{mendelzon-simplepath} show that the regular simple path problem is \NP-complete in the general case. 
However, they show that the problem can be decided in polynomial time 
for subword-closed languages. 
They also show that the problem becomes polynomial under some restrictions 
on the size of cycles of both graph and automaton. 
A subsequent paper~\cite{nedev00} proves the polynomiality for the class of outerplanar graphs. 
Barrett et al.~\cite{barrett-simplepath} extend this result, proving that the regular simple path problem 
is polynomial w.r.t. combined complexity for graphs of bounded treewidth.
Let us also observe that the existence of a regular simple path between two vertices is MSO-definable, 
and therefore a well-known result of Courcelle~\cite{mso-courcelle} already
implies the same result but w.r.t. data complexity only.
Barrett et al.~\cite{barrett-simplepath} also show that the problem is \NP-complete for the class of grid graphs
even when the language is fixed. Practical algorithms for regular simple paths on large graphs have been proposed in~\cite{JinHWRX10,leser-largegraphs}.

Regular simple paths have been also investigated in the context of SPARQL property paths with the semantics
proposed in a working draft of SPARQL 1.1. 
Notice that such semantics of SPARQL property paths doesn't exactly correspond to regular simple paths queries.
Losemann and Martens~\cite{losemann-sparql} and Arenas et al.~\cite{arenas-counting}
investigate the complexity of evaluating such property paths.
They show that the evaluation is \NP-complete in several cases, along with exhibiting cases in which it is polynomial.
More precisely, Losemann and Martens consider different fragments of regular expressions and classify them with respect to
the complexity of evaluating SPARQL property paths. Both papers also show that counting the number of paths
that match a regular expression (which is permitted by the working draft) is hard in many cases.


